Second-Order Neural ODE Optimizer

We propose a novel second-order optimization framework for training the emerging deep continuous-time models, specifically the Neural Ordinary Differential Equations (Neural ODEs). Since their training already involves expensive gradient computation by solving a backward ODE, deriving efficient second-order methods becomes highly nontrivial. Nevertheless, inspired by the recent Optimal Control (OC) interpretation of training deep networks, we show that a specific continuous-time OC methodology, called Differential Programming, can be adopted to derive backward ODEs for higher-order derivatives at the same O(1) memory cost. We further explore a low-rank representation of the second-order derivatives and show that it leads to efficient preconditioned updates with the aid of Kronecker-based factorization. The resulting method -- named SNOpt -- converges much faster than first-order baselines in wall-clock time, and the improvement remains consistent across various applications, e.g. image classification, generative flow, and time-series prediction. Our framework also enables direct architecture optimization, such as the integration time of Neural ODEs, with second-order feedback policies, strengthening the OC perspective as a principled tool of analyzing optimization in deep learning. Our code is available at https://github.com/ghliu/snopt.

==> subtex/checklist.tex <==


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{This paper concerns general optimization with theoretical analysis using OCP. Hence, we believe the societal impact is not directly applicable.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
    \item Did you include complete proofs of all theoretical results?
    \answerYes{In Appendix~\ref{app:2} and \ref{app:3}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{In Appendix~\ref{app:4}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In Appendix~\ref{app:4}.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In Appendix~\ref{app:4}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Table~\ref{table:F-config}.}
  \item Did you mention the license of the assets?
    \answerYes{See Table~\ref{table:F-config}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> subtex/math_commands2.tex <==



\newcommand{\rpartial}{{\mathrm{\partial}}}
\newcommand{\rinf}{{\mathrm \inf}}
\newcommand{\rd}{{\mathrm d}}

\newcommand{\rp}{{\mathrm p}}
\newcommand{\re}{{\mathrm e}}
\newcommand{\rdelta}{{\mathrm \delta}}
\newcommand{\rtr}{{\mathrm{tr}}}
\newcommand{\rP}{{\mathrm{P}}}
\newcommand{\rT}{{\mathrm{T}}}
\newcommand{\rvec}{{\mathrm{vec}}}
\newcommand{\rtau}{{\mathrm{\tau}}}


\newcommand{\vxi}{{\mbox{\boldmath$\xi$}}}
\newcommand{\vpi}{{\mbox{\boldmath$\pi$}}}
\newcommand{\vdomega}{{\bf d\omega}}
\newcommand{\vlambda}{{\mbox{\boldmath$\lambda$}}}
\newcommand{\vBamma}{{\mbox{\boldmath$\Gamma$}}}
\newcommand{\VTheta}{{\mbox{\boldmath$\Theta$}}}
\newcommand{\vPhi}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\vphi}{{\mbox{\boldmath$\phi$}}}
\newcommand{\vPsi}{{\mbox{\boldmath$\Psi$}}}
\newcommand{\ve}{{\mbox{\boldmath$\epsilon$}}}
\newcommand{\vSigma}{{\mbox{\boldmath$\Sigma$}}}
\newcommand{\valpha}{{\mbox{\boldmath$\alpha$}}}
\newcommand{\vmu}{{\mbox{\boldmath$\mu$}}}
\newcommand{\vbeta}{{\mbox{\boldmath$\beta$}}}
\newcommand{\vomega}{{\mbox{\boldmath$\omega$}}}
\newcommand{\vtau}{{\mbox{\boldmath$\tau$}}}
\newcommand{\vdtau}{{\mbox{\boldmath$d\tau$}}}
\newcommand{\vtheta}{{\mbox{\boldmath$\theta$}}}\newcommand{\dataset}{{\cal D}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calE}{{\cal E}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calI}{{\cal I}}
\newcommand{\calJ}{{\cal J}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calL}{{\cal L}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\calO}{{\cal O}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calT}{{\cal T}}
\newcommand{\calU}{{\cal U}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calW}{{\cal W}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}
\newcommand{\calZ}{{\cal Z}}

\newcommand{\vcalA}{{\mbox{\boldmath$\cal{A}$}}}
\newcommand{\vcalB}{{\mbox{\boldmath$\cal{B}$}}}
\newcommand{\vcalC}{{\mbox{\boldmath$\cal{C}$}}}
\newcommand{\vcalD}{{\mbox{\boldmath$\cal{D}$}}}
\newcommand{\vcalE}{{\mbox{\boldmath$\cal{E}$}}}
\newcommand{\vcalF}{{\mbox{\boldmath$\cal{F}$}}}
\newcommand{\vcalG}{{\mbox{\boldmath$\cal{G}$}}}
\newcommand{\vcalH}{{\mbox{\boldmath$\cal{H}$}}}
\newcommand{\vcalI}{{\mbox{\boldmath$\cal{I}$}}}
\newcommand{\vcalJ}{{\mbox{\boldmath$\cal{J}$}}}
\newcommand{\vcalK}{{\mbox{\boldmath$\cal{K}$}}}
\newcommand{\vcalL}{{\mbox{\boldmath$\cal{L}$}}}
\newcommand{\vcalM}{{\mbox{\boldmath$\cal{M}$}}}
\newcommand{\vcalN}{{\mbox{\boldmath$\cal{N}$}}}
\newcommand{\vcalO}{{\mbox{\boldmath$\cal{O}$}}}
\newcommand{\vcalP}{{\mbox{\boldmath$\cal{P}$}}}
\newcommand{\vcalQ}{{\mbox{\boldmath$\cal{Q}$}}}
\newcommand{\vcalR}{{\mbox{\boldmath$\cal{R}$}}}
\newcommand{\vcalS}{{\mbox{\boldmath$\cal{S}$}}}
\newcommand{\vcalT}{{\mbox{\boldmath$\cal{T}$}}}
\newcommand{\vcalU}{{\mbox{\boldmath$\cal{U}$}}}
\newcommand{\vcalV}{{\mbox{\boldmath$\cal{V}$}}}
\newcommand{\vcalW}{{\mbox{\boldmath$\cal{W}$}}}
\newcommand{\vcalX}{{\mbox{\boldmath$\cal{X}$}}}
\newcommand{\vcalY}{{\mbox{\boldmath$\cal{Y}$}}}
\newcommand{\vcalZ}{{\mbox{\boldmath$\cal{Z}$}}}



\newcommand{\vcalg}{{\mbox{\boldmath$\cal{g}$}}}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\fracdiff}[2]{\frac{\rd #1}{\rd  #2}}

\newcommand{\T}{\mathsf{T}}


\newcommand{\Xspace}{\mathcal{X}}
\newcommand{\snew}{\mathbf{x}^\prime}
\newcommand{\s}{\mathbf{x}}
\newcommand{\Pas}[2]{\mathcal{P}\left({#1}|{#2}\right)}
\newcommand{\Pol}[2]{\mathcal{U}\left({#1}|{#2}\right)}
\newcommand{\PolOpt}[2]{\mathcal{U}^{*}\left({#1}|{#2}\right)}
\newcommand{\PolPasT}[1]{\mathcal{P}\left({#1}\right)}
\newcommand{\PolT}[1]{\mathcal{U}\left({#1}\right)}
\newcommand{\traj}{\mathbf{X}}
\newcommand{\costt}[1]{\mathcal{J}\left({#1}\right)}
\newcommand{\logb}[1]{\log\left({#1}\right)}
\newcommand{\expb}[1]{\exp\left({#1}\right)}
\newcommand{\val}[2]{\mathit{V}_{#2}\left({#1}\right)}
\newcommand{\zt}[2]{\Phi_{#2}\left({#1}\right)}
\newcommand{\nZ}[2]{\mathcal{G}_t[\Phi]\left({#1}\right)}
\newcommand{\ExP}[2]{\E_{{#1}}{\left[#2\right]}}







\newcommand{\vTheta}{{\mbox{\boldmath$\Theta$}}}
\newcommand{\vUpsilon}{{\mbox{\boldmath$\Upsilon$}}}

\newcommand{\VOmega}{{\mbox{\boldmath$\Omega$}}}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}%



\newcommand{\vzeta}{{\bf \zeta}}
\newcommand{\veta}{{\bf \eta}}

\newcommand{\Langle}{{\Big\langle}}
\newcommand{\Rangle}{{\Big\rangle}}






\makeatletter
\newcommand{\vast}{\bBigg@{3.5}}
\newcommand{\Vast}{\bBigg@{4}}
\newcommand{\vastt}{\bBigg@{4.5}}
\newcommand{\Vastt}{\bBigg@{5}}
\makeatother

\newcommand{\beginsupplement}{
        \setcounter{table}{0}
        \renewcommand{\thetable}{S\arabic{table}}
        \setcounter{figure}{0}
        \renewcommand{\thefigure}{S\arabic{figure}}
        \setcounter{section}{0}
        \renewcommand{\thesection}{S\arabic{section}}
        \setcounter{equation}{0}
        \renewcommand{\theequation}{S\arabic{equation}}
        \setcounter{algorithm}{0}
        \renewcommand{\thealgorithm}{S\arabic{algorithm}}
     }



\newcommand{\VS}{{~\emph{v.s.}~}}

\newcommand{\br}[1]{\left[#1\right]}
\newcommand{\pr}[1]{\left(#1\right)}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\abs}[1]{\left|#1\right|}


\newcommand*\bvec[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bmat}[4]{\begin{bmatrix} #1 & #2 \\ #3 & #4\end{bmatrix}}

